SUGAR: Leveraging Contextual Confidence for Smarter Retrieval

Bearing in mind the limited parametric knowledge of Large Language Models (LLMs), retrieval-augmented generation (RAG) which supplies them with the relevant external knowledge has served as an approach to mitigate the issue of hallucinations to a certain extent. However, uniformly retrieving supporting context makes response generation source-inefficient, as triggering the retriever is not always necessary, or even inaccurate, when a model gets distracted by noisy retrieved content and produces an unhelpful answer. Motivated by these issues, we introduce Semantic Uncertainty Guided Adaptive Retrieval (SUGAR), where we leverage context-based entropy to actively decide whether to retrieve and to further determine between single-step and multi-step retrieval. Our empirical results show that selective retrieval guided by semantic uncertainty estimation improves the performance across diverse question answering tasks, as well as achieves a more efficient inference.

==> name.tex <==
\begin{table*}[h!]
\caption{Experiment results on Single-hop and Multi-hop QA datasets.}
\label{tab:table1}
\normalsize
\resizebox{\textwidth}{!}{
\begin{tabular}{lllllllllllllllllllllll}
\toprule
\multirow{2}{*}{Data} & \multirow{2}{*}{Types} & \multirow{2}{*}{Methods} & \multicolumn{5}{c}{SQuAD} & \multicolumn{5}{c}{Natural Questions} & \multicolumn{5}{c}{TriviaQA} \\ \cmidrule(r){4-18}
& & & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Step} & \multicolumn{1}{c}{Time} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Step} & \multicolumn{1}{c}{Time} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Step} & \multicolumn{1}{c}{Time} \\ \midrule

\multirow{8}{*}{Single-hop} 
& \multirow{2}{*}{Simple} & No Retrieval & 3.60 & 10.50 & 5.00 & 0.00 & 0.11 & 14.20 & 19.00 & 15.60 & 0.00 & 0.13 & 25.00 & 31.80 & 27.00 & 0.00 & 0.13 \\
& & Single-step Approach & 27.80 & 39.30 & 34.00 & 1.00 & 1.00 & 37.80 & 47.30 & 44.60 & 1.00 & 1.00 & 53.60 & 62.40 & 60.20 & 1.00 & 1.00 \\ \cmidrule(r){2-18}

& \multirow{4}{*}{Adaptive} & Adaptive Retrieval \cite{C4} & 13.40 & 23.10 & 17.60 & 0.50 & 0.55 & 28.20 & 36.00 & 33.00 & 0.50 & 0.56 & 38.40 & 46.90 & 42.60 & 0.50 & 0.56 \\
& & Self-RAG \cite{C13} & 2.20 & 11.20 & 18.40 & 0.63 & 0.50 & 31.40 & 39.00 & 33.60 & 0.63 & 0.17 & 12.80 & 29.30 & 57.00 & 0.68 & 0.45 \\
& & Adaptive-RAG \cite{C6} & 26.80 & 38.30 & 33.00 & 1.37 & 2.02 & 37.80 & 47.30 & 44.60 & 1.00 & 1.00 & 52.20 & 60.70 & 58.20 & 1.23 & 1.54 \\
& & SUGAR (Ours) & \textbf{34.50} & \textbf{47.19} & \textbf{53.50} & \textbf{1.23} & 4.43 & 31.75 & 41.30 & \textbf{46.25} & \textbf{1.00} & \textbf{1.00}  & \textbf{55.75} & \textbf{64.25} & \textbf{69.25} & \textbf{0.77} & 3.13 \\ \cmidrule(r){2-18}

& \multirow{1}{*}{Complex} & Multi-step Approach \cite{C23} & 24.40 & 35.60 & 29.60 & 4.52 & 9.03 & 38.60 & 47.80 & 44.20 & 5.04 & 10.18 & 53.80 & 62.40 & 60.20 & 5.28 & 9.22 \\ \midrule

\multirow{8}{*}{Datasets}
& & & \multicolumn{5}{c}{MuSiQue} & \multicolumn{5}{c}{HotpotQA} & \multicolumn{5}{c}{2WikiMultiHopQA} \\ \cmidrule(r){4-18}
& & & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Step} & \multicolumn{1}{c}{Time} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Step} & \multicolumn{1}{c}{Time} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{Step} & \multicolumn{1}{c}{Time} \\ \midrule

\multirow{8}{*}{Multi-hop} 
& \multirow{2}{*}{Simple} & No Retrieval & 2.40 & 10.70 & 3.20 & 0.00 & 0.11 & 16.60 & 22.71 & 17.20 & 0.00 & 0.11 & 27.40 & 32.04 & 27.80 & 0.00 & 0.10 \\
& & Single-step Approach & 13.80 & 22.80 & 15.20 & 1.00 & 1.00 & 34.40 & 46.15 & 36.40 & 1.00 & 1.00 & 41.60 & 47.90 & 42.80 & 1.00 & 1.00 \\ \cmidrule(r){2-18}

& \multirow{4}{*}{Adaptive} & Adaptive Retrieval \cite{C4} & 6.40 & 15.80 & 8.00 & 0.50 & 0.55 & 23.60 & 32.22 & 25.00 & 0.50 & 0.55 & 33.20 & 39.44 & 34.20 & 0.50 & 0.55 \\
& & Self-RAG \cite{C13} & 1.60 & 8.10 & 12.00 & 0.73 & 0.51 & 6.80 & 17.53 & 29.60 & 0.73 & 0.45 & 4.60 & 19.59 & 38.80 & 0.93 & 0.49 \\
% & & Adaptive-RAG & 23.60 & 31.80 & 26.00 & 3.22 & 6.61 & 42.00 & 53.82 & 44.40 & 3.55 & 5.99 & 40.60 & 49.75 & 46.40 & 2.63 & 4.68 \\
& & SUGAR (Ours) & & & & & & \textbf{38.77} & \textbf{49.85} & \textbf{50.25} & \textbf{2.31} & \textbf{5.11} & \textbf{25.00} & \textbf{41.92} & \textbf{39.75} & \textbf{0.88} & \textbf{4.86} \\ \cmidrule(r){2-18}

& \multirow{1}{*}{Complex} & Multi-step Approach \cite{C23} & 23.00 & 31.90 & 25.80 & 3.60 & 7.58 & 44.60 & 56.54 & 47.00 & 5.53 & 9.38 & 49.60 & 58.85 & 55.40 & 4.17 & 7.37 \\ \bottomrule

\end{tabular}
}
\end{table*}

